Croppable Knowledge Graph Embedding

Knowledge Graph Embedding (KGE) is a common approach for Knowledge Graphs (KGs) in AI tasks. Embedding dimensions depend on application scenarios. Requiring a new dimension means training a new KGE model from scratch, increasing cost and limiting efficiency and flexibility. In this work, we propose a novel KGE training framework MED. It allows one training to obtain a croppable KGE model for multiple scenarios with different dimensional needs. Sub-models of required dimensions can be directly cropped and used without extra training. In MED, we propose a mutual learning mechanism to improve the low-dimensional sub-models and make high-dimensional sub-models retain the low-dimensional sub-models' capacity, an evolutionary improvement mechanism to promote the high-dimensional sub-models to master the triple that the low-dimensional sub-models can not, and a dynamic loss weight to adaptively balance the multiple losses. Experiments on 4 KGE models across 4 standard KG completion datasets, 3 real-world scenarios using a large-scale KG, and extending MED to the BERT language model demonstrate its effectiveness, high efficiency, and flexible extensibility.

==> table/table-FB15K237-hit1_3.tex <==
\setlength\tabcolsep{4pt}%列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[ht]
\caption{Hit@1 and Hit@3 of some representative dimensions on FB15K237.}
\label{table_FB15K237_hit1_3}
\begin{center}
    \resizebox{.9\textwidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c}{\textbf{}}                      & \multicolumn{2}{c}{\textbf{10d}} & \multicolumn{2}{c}{\textbf{20d}} & \multicolumn{2}{c}{\textbf{40d}} & \multicolumn{2}{c}{\textbf{80d}} & \multicolumn{2}{c}{\textbf{160d}} & \multicolumn{2}{c}{\textbf{320d}} & \multicolumn{2}{c}{\textbf{640d}} \\
\midrule
\multirow{9}{*}{\textbf{TransE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16} 
                                 & DT              & .169           & .102          & .301           & .190           & .327           & .212          & .340            & .218          & .348           & .222           & .353           & .224           & \textbf{.358}  & \textbf{.228}  \\
                                 & Ext             & .123           & .065          & .211           & .122          & .264           & .156          & .296           & .180           & .320            & .197           & .331           & .208           & .358           & .228           \\
                                 & Ext-L           & .118           & .065          & .192           & .115          & .256           & .157          & .292           & .180           & .316           & .198           & .333           & .210            & .358           & .228           \\
                                 & Ext-V           & .150            & .081          & .222           & .126          & .265           & .156          & .301           & .185          & .325           & .205           & .341           & .217           & .358           & .228           \\
                                 & BKD             & .178           & .106          & .308           & .198          & .336           & .208          & .349           & .222          & .349           & .223           & .354           & .226           & -               & -               \\
                                 & TA              & .188           & .112          & .307           & .200            & .336           & .212          & .348           & .220           & .353           & .225           & .355           & .223           & -               & -               \\
                                 & DualDE          & .193           & .115           & .307           & \textbf{.201} & .337           & .216          & \textbf{.351}  & .223          & \textbf{.354}  & .226           & \textbf{.356}  & \textbf{.227}  & -               & -               \\
                                 & {\model}            & \textbf{.215}  & \textbf{.122} & \textbf{.321}  & .199          & \textbf{.338}  & \textbf{.218} & .347           & \textbf{.223} & .351           & .226           & \textbf{.356}  & .227           & .358           & .227           \\
                                 %\midrule
                                 %\multirow{9}{*}{\textbf{SimplE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}   & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16}
                         %        & DT              & .103           & .055          & .193           & .105          & .256           & .161          & .297           & .191          & .314           & .197           & .323            & .208          & \textbf{.324}  & \textbf{.211}  \\
                       %          & Ext             & .039           & .019          & .071           & .047          & .091           & .057          & .171           & .109          & .251           & .159           & .294            & .187          & .324           & .211           \\
                       %          & Ext-L           & .043           & .035          & .048           & .037          & .111           & .040          & .131           & .093          & .216           & .134           & .281            & .177          & .324           & .211           \\
                         %        & Ext-V           & .047           & .036          & .074           & .043          & .097           & .077          & .145           & .109          & .248           & .156           & .289            & .189          & .324           & .211           \\
                        %         & BKD             & .123           & .064          & .201           & .115          & .261           & .164          & .299           & .191          & .308           & .202           & .318            & \textbf{.213} & -               & -               \\
                        %         & TA              & .133           & .073          & .210           & .123          & .276           & .175          & .302           & .195          & .318           & .203           & .323            & .211          & -               & -               \\
                       %          & DualDE          & .130           & .071          & .224           & .115          & .279           & .175          & .305           & .196          & \textbf{.324}  & \textbf{.208}  & \textbf{,.326}  & .211          & -               & -               \\
                       %          & {\model}        & \textbf{.164}  & \textbf{.073} & \textbf{.254}  & \textbf{.158} & \textbf{.288}  & \textbf{.177} & \textbf{.305}  & \textbf{.196} & .319           & .205           & .318            & .208          & .321           & .207           \\
                                 \midrule
\multirow{9}{*}{\textbf{RotatE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16} 
                                 & DT              & .284           & .168          & .330            & .207          & .346           & .223          & .352           & .224          & .353           & .229           & .357           & .230            & \textbf{.363}  & \textbf{.234}  \\
                                 & Ext             & .152           & .080           & .225           & .129          & .278           & .170           & .304           & .190           & .322           & .203           & .335           & .217           & .363           & .234           \\
                                 & Ext-L           & .147           & .078          & .209           & .121          & .247           & .146          & .275           & .166          & .312           & .193           & .333           & .209           & .363           & .234           \\
                                 & Ext-V           & .174           & .097          & .218           & .126          & .264           & .159          & .293           & .182          & .319           & .201           & .336           & .213           & .363           & .234           \\
                                 & BKD             & .306           & .193          & .338           & .214          & .352           & .224          & .354           & .230           & .356           & .230            & .358           & .231           & -               & -               \\
                                 & TA              & .308           & .196          & .339           & .216          & .353           & .225          & .358           & .229          & .359           & .229           & .358           & .231           & -               & -               \\
                                 & DualDE          & .311           & .197          & .341           & .216          & .353           & \textbf{.227} & \textbf{.360}   & .230           & \textbf{.361}  & .232           & .361           & \textbf{.233}  & -               & -               \\
                                 & {\model}            & \textbf{.324}  & \textbf{.201} & \textbf{.344}  & \textbf{.216} & \textbf{.355}  & .225          & .357           & \textbf{.231} & .358           & \textbf{.233}  & \textbf{.362}  & \textbf{.233}  & .362           & .232 \\
                                 \midrule
                                 \multirow{9}{*}{\textbf{PairRE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}   & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16}
                                 & DT              & .198           & .116          & .262           & .162          & .312           & .202          & .337           & .222          & .352           & .227           & .364            & .235          & \textbf{.368}  & \textbf{.237}  \\
                                 & Ext             & .158           & .107          & .187           & .118          & .236           & .149          & .283           & .182          & .325           & .207           & .354            & .230          & .368           & .237           \\
                                 & Ext-L           & .159           & .099          & .196           & .134          & .238           & .159          & .298           & .188          & .342           & .219           & .359            & .233          & .368           & .237           \\
                                 & Ext-V           & .181           & .116          & .192           & .125          & .250           & .154          & .307           & .193          & .343           & .221           & .362            & .237          & .368           & .237           \\
                                 & BKD             & .215           & .132          & .265           & .168          & .314           & .203          & .343           & .224          & .355           & .233           & .366            & .236          & -               & -               \\
                                 & TA              & .226           & .139          & .291           & .182          & .316           & .210          & .347           & .224          & .358           & .232           & .368            & .235          & -               & -               \\
                                 & DualDE          & .224           & .139          & .286           & .179          & .318           & .212          & \textbf{.351}  & \textbf{.226} & \textbf{.359}  & \textbf{.234}  & \textbf{.371}   & \textbf{.238} & -               & -               \\
                                 & {\model}        & \textbf{.253}  & \textbf{.172} & \textbf{.299}  & \textbf{.189} & \textbf{.327}  & \textbf{.213} & .346           & .224          & .357           & .232           & .366            & .236          & .368           & .235          \\
                                 \bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> table/table-FB15K327.tex <==
\setlength\tabcolsep{4pt}%调列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[ht]
\caption{MRR and Hit@10 of some representative dimensions on FB15K237.}\label{table_FB15K237}
\begin{center}
\resizebox{.9\textwidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c}{\textbf{}}                      & \multicolumn{2}{c}{\textbf{10d}} & \multicolumn{2}{c}{\textbf{20d}} & \multicolumn{2}{c}{\textbf{40d}} & \multicolumn{2}{c}{\textbf{80d}} & \multicolumn{2}{c}{\textbf{160d}} & \multicolumn{2}{c}{\textbf{320d}} & \multicolumn{2}{c}{\textbf{640d}} \\
\midrule
\multirow{9}{*}{\textbf{TransE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\ \cline{2-16}
                                 & DT              & .150           & .235           & .277          & .440            & .299          & .477           & .313          & .484           & .315           & .499           & .318           & .501           & .322           & \textbf{.508}  \\
                                 & Ext             & .115          & .211           & .191          & .324           & .236          & .392           & .266          & .436           & .286           & .462           & .299           & .479           & .322           & .508           \\
                                 & Ext-L          & .109          & .194           & .175          & .293           & .232          & .381           & .263          & .424           & .285           & \textbf{.462}  & .301           & .484           & .322           & .508           \\
                                 & Ext-V          & .139          & .256           & .200            & .348           & .237          & .396           & .270           & .437           & .293           & .466           & .308           & .488           & .322           & .508           \\
                                 & BKD             & .176          & .293           & .279          & .446           & .303          & .480            & .315          & .500            & .315           & .501           & .320            & .502           & -               & -               \\
                                 & TA              & .175          & .246           & .281          & .441           & .303          & .484           & .314          & .498           & .319           & .504           & .321           & .504           & -               & -               \\
                                 & DualDE          & .179          & .301           & .281          & .443           & .306          & .483           & .316          & \textbf{.502}  & .319           & .505           & \textbf{.322}  & \textbf{.508}  & -               & -               \\
                                 & {\model}           & \textbf{.196} & \textbf{.341}  & \textbf{.290}  & \textbf{.472}  & \textbf{.308} & \textbf{.486}  & \textbf{.317} & .502           & \textbf{.320}   & \textbf{.505}  & .321           & .507           & \textbf{.322}  & .507           \\
                                % \midrule
                                 %\multirow{9}{*}{\textbf{SimplE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\ \cline{2-16}
                          %       & DT              & .097          & .179           & .176          & .321           & .236          & .390           & .271          & .431           & .285           & .458           & .291           & .467           & \textbf{.295}  & \textbf{.472}  \\
                          %       & Ext             & .037          & .068           & .069          & .107           & .090          & .144           & .159          & .258           & .229           & .372           & .269           & .432           & .295           & .472           \\
                        %         & Ext-L           & .045          & .059           & .056          & .062           & .083          & .146           & .114          & .205           & .196           & .316           & .258           & .421           & .295           & .472           \\
                        %         & Ext-V           & .049          & .069           & .066          & .101           & .105          & .149           & .138          & .224           & .224           & .369           & .261           & .414           & .295           & .472           \\
                        %         & BKD             & .113          & .204           & .182          & .315           & .244          & .412           & .275          & .439           & .287           & .463           & .293           & .470           & -               & -               \\
                       %          & TA              & .124          & .221           & .192          & .329           & .254          & .416           & .276          & .448           & .290           & .465           & .295           & .471           & -               & -               \\
                       %          & DualDE          & .120          & .213           & .195          & .346           & .258          & \textbf{.429}  & .279          & .443           & \textbf{.293}  & .466           & \textbf{.296}  & \textbf{.468}  & -               & -               \\
                    %             & {\model}        & \textbf{.143} & \textbf{.267}  & \textbf{.233} & \textbf{.384}  & \textbf{.261} & .427           & \textbf{.279} & \textbf{.448}  & .291           & \textbf{.466}  & .293           & .466           & .293           & .468           \\
                                 \midrule
\multirow{9}{*}{\textbf{RotatE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\ \cline{2-16}
                                 & DT              & .254          & .424           & .297          & .477           & .312          & .495           & .317          & .502           & .322           & .506           & .323           & .510            & \textbf{.325}  & \textbf{.515}  \\
                                 & Ext             & .138          & .245           & .203          & .340            & .251          & .410            & .276          & .443           & .291           & .465           & .305           & .485           & .325           & .515           \\
                                 & Ext-L          & .135          & .243           & .188          & .319           & .221          & .365           & .246          & .402           & .280            & .453           & .299           & .477           & .325           & .515           \\
                                 & Ext-V          & .160           & .281           & .198          & .340            & .238          & .393           & .265          & .427           & .288           & .458           & .302           & .478           & .325           & .515           \\
                                 & BKD             & .277          & .442           & .305          & .485           & .314          & .503           & .321          & .508           & .322           & .510            & .323           & .509           & -               & -               \\
                                 & TA              & .280           & .447           & .306          & .485           & .313          & .501           & .319          & .507           & \textbf{.323}  & .510            & .323           & .509           & -               & -               \\
                                 & DualDE          & .282          & .449           & .307          & .486           & .315          & .502           & .318          & .507           & .322           & \textbf{.512}  & .324           & \textbf{.514}  & -               & -               \\
                                 & {\model}           & \textbf{.288} & \textbf{.459}  & \textbf{.311} & \textbf{.492}  & \textbf{.318} & \textbf{.504}  & \textbf{.322} & \textbf{.509}  & \textbf{.323}  & .510            & \textbf{.324}  & .512           & .324           & .514          
\\ \midrule
\multirow{9}{*}{\textbf{PairRE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\ \cline{2-16}
                                 & DT              & .182          & .314           & .243          & .395           & .284          & .452           & .307          & .476           & .319           & .505           & .328           & .518           & \textbf{.332}  & \textbf{.522}  \\
                                 & Ext             & .148          & .222           & .177          & .289           & .217          & .353           & .259          & .416           & .294           & .469           & .321           & .506           & .332           & .522           \\
                                 & Ext-L           & .150          & .249           & .196          & .294           & .219          & .333           & .271          & .436           & .309           & .489           & .326           & .513           & .332           & .522           \\
                                 & Ext-V           & .176          & .277           & .192          & .303           & .229          & .374           & .279          & .450           & .311           & .490           & .329           & .513           & .332           & .522           \\
                                 & BKD             & .198          & .332           & .251          & .407           & .288          & .453           & .311          & .487           & .321           & .508           & .330           & .521           & -               & -               \\
                                 & TA              & .208          & .346           & .263          & .430           & .292          & .455           & .314          & .493           & .323           & .509           & .332           & .521           & -               & -               \\
                                 & DualDE          & .207          & .342           & .261          & .427           & .293          & .456           & \textbf{.316} & .495           & \textbf{.326}  & \textbf{.512}  & \textbf{.334}  & \textbf{.524}  & -               & -               \\
                                 & {\model}        & \textbf{.239} & \textbf{.384}  & \textbf{.274} & \textbf{.437}  & \textbf{.303} & \textbf{.466}  & .314          & \textbf{.495}  & .324           & .510           & .329           & .521           & .330           & .520          \\

\bottomrule
\end{tabular}
}    
\end{center}

\end{table*}


==> table/table-WN18RR-hit1_3.tex <==
\setlength\tabcolsep{4pt}%调列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[ht]
\caption{Hit@1 and Hit@3 of some representative dimensions on WN18RR.}\label{table_WN18RR_hit1_3}
\begin{center}
    \resizebox{.9\textwidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c}{\textbf{}}                      & \multicolumn{2}{c}{\textbf{10d}} & \multicolumn{2}{c}{\textbf{20d}} & \multicolumn{2}{c}{\textbf{40d}} & \multicolumn{2}{c}{\textbf{80d}} & \multicolumn{2}{c}{\textbf{160d}} & \multicolumn{2}{c}{\textbf{320d}} & \multicolumn{2}{c}{\textbf{640d}} \\
\midrule
\multirow{9}{*}{\textbf{TransE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16} 
                                 & DT              & .202           & .011          & .291           & .016          & .385           & .018          & .401           & .025          & .403           & .027           & .407           & .033           & .412           & \textbf{.034}  \\
                                 & Ext             & .201           & .016          & .285           & .023          & .338           & .023          & .364           & .028          & .384           & .033           & .388           & .028           & .412           & .034           \\
                                 & Ext-L           & .218           & .029          & .317           & .025          & .361           & .039          & .403           & .046          & .405           & .036           & .408           & .033           & .412           & .034           \\
                                 & Ext-V           & .218           & .029          & .314           & \textbf{.045} & .391           & \textbf{.051} & .407           & \textbf{.047} & .408           & .036           & .411           & .027           & .412           & .034           \\
                                 & BKD             & .216           & .035          & .331           & .040           & .392           & .033          & .401           & .031          & .404           & .030            & .407           & .032           & -               & -               \\
                                 & TA              & .224           & .040           & .343           & .043          & .395           & .037          & .408           & .030           & .407           & .030            & .410            & .034           & -               & -               \\
                                 & DualDE          & .226           & .037          & .346           & .043          & .394           & .037          & \textbf{.408}  & .031          & \textbf{.408}  & .031           & \textbf{.411}  & \textbf{.034}  & -               & -               \\
                                 & {\model}            & \textbf{.269}  & \textbf{.040}  & \textbf{.369}  & \textbf{.045} & \textbf{.399}  & .038          & .404           & .042          & .407           & \textbf{.037}  & .410            & .033           & \textbf{.412}  & .031           \\
                                 %\midrule
                                 %\multirow{9}{*}{\textbf{SimplE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\
                                 
%\cline{2-16}                     
%& DT              & .061           & .028          & .297           & .193          & .361           & .289          & .406           & .343          & .420           & .382           & .428           & .386           & .433           & \textbf{.391}  \\
                                 %& Ext             & .003           & .001          & .055           & .023          & .181           & .114          & .249           & .168          & .377           & .329           & .422           & .381           & .433           & .391           \\
                               %  & Ext-L           & .004           & .003          & .051           & .031          & .187           & .128          & .389           & .333          & .413           & .365           & .429           & .384           & .433           & .391           \\
                             %    & Ext-V           & .004           & .002          & .050           & .029          & .269           & .205          & .378           & .349          & .409           & .372           & .426           & .382           & .433           & .391           \\
                           %      & BKD             & .077           & .034          & .331           & .225          & .384           & .311          & .415           & .358          & .426           & .371           & .431           & .385           & -               & -               \\
                           %      & TA              & .093           & .042          & .349           & .269          & .380           & .349          & .412           & \textbf{.384} & .425           & .388           & .431           & .389           & -               & -               \\
                      %           & DualDE          & .086           & .038          & .361           & .285          & .391           & \textbf{.368} & .416           & .383          & .427           & \textbf{.389}  & \textbf{.434}  & \textbf{.392}  & -               & -               \\
              %                   & {\model}        & \textbf{.119}  & \textbf{.048} & \textbf{.366}  & \textbf{.292} & \textbf{.395}  & .359          & \textbf{.419}  & .380          & \textbf{.428}  & .389           & .434           & .390           & \textbf{.434}  & .388           \\
                                 \midrule
\multirow{9}{*}{\textbf{RotatE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16} 
                                 & DT              & .304           & .005          & .436           & .357          & .475           & .393          & .487           & .420           & .489           & .423           & .491           & .428           & .493           & \textbf{.429}  \\
                                 & Ext             & .315           & .257          & .399           & .335          & .452           & .395          & .472           & .415          & .480            & .413           & .470            & .418           & .493           & .429           \\
                                 & Ext-L           & .224           & .166          & .359           & .288          & .420            & .352          & .441           & .373          & .461           & .396           & .481           & .417           & .493           & .429           \\
                                 & Ext-V           & .289           & .197          & .336           & .234          & .377           & .263          & .402           & .293          & .442           & .357           & .467           & .397           & .493           & .429           \\
                                 & BKD             & .312           & .009          & .452           & .361          & .479           & .403          & .487           & .421          & .490            & .424           & .492           & .425           & -               & -               \\
                                 & TA              & .314           & .010           & .452           & .363          & .481           & .408          & .489           & .420           & .488           & .422           & .492           & .425           & -               & -               \\
                                 & DualDE          & .320            & .011          & .452           & .364          & .483           & .412          & .489           & \textbf{.423} & .488           & \textbf{.426}  & .491           & .425           & -               & -               \\
                                 & {\model}            & \textbf{.354}  & \textbf{.277} & \textbf{.476}  & \textbf{.409} & \textbf{.486}  & \textbf{.418} & \textbf{.490}   & .422          & \textbf{.492}  & .424           & \textbf{.493}  & \textbf{.427}  & \textbf{.495}  & .428  \\
                                 \midrule
                                 \multirow{9}{*}{\textbf{PairRE}} & \textit{Method} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1} & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  & \textit{Hit@3}  & \textit{Hit@1}  \\ \cline{2-16}
                                 & DT              & .271           & .174         & .368           & .313          & .428           & .384          & .450           & .399          & .463           & .405           & .462           & .406           & \textbf{.464}  & \textbf{.407}  \\
                                 & Ext             & .163           & .120          & .292           & .198          & .366           & .267          & .398           & .314          & .437           & .364           & .452           & .388           & .464           & .407           \\
                                 & Ext-L           & .175           & .129          & .302           & .237          & .383           & .319          & .431           & .377          & .450           & .395           & .455           & .400           & .464           & .407           \\
                                 & Ext-V           & .192           & .124          & .323           & .269          & .407           & .352          & .435           & .379          & .452           & .398           & .458           & .400           & .464           & .407           \\
                                 & BKD             & .279           & .184          & .388           & .334          & .435           & .372          & .452           & .405          & .460           & .405           & .463           & .407           & -               & -               \\
                                 & TA              & .293           & .197          & .387           & .332          & .437           & .380          & .460           & .404          & .462           & .409           & .463           & .408           & -               & -               \\
                                 & DualDE          & .281           & .175          & .389           & .330          & .437           & .381          & \textbf{.463}  & \textbf{.409} & .463           & \textbf{.410}  & .465           & \textbf{.410}  & -               & -               \\
                                 & {\model}        & \textbf{.314}  & \textbf{.259} & \textbf{.426}  & \textbf{.367} & \textbf{.443}  & \textbf{.392} & .462           & .405          & \textbf{.464}  & .406           & \textbf{.465}  & .407           & .464           & .406          \\
                                 \bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> table/table-WN18RR.tex <==
\setlength\tabcolsep{4pt}%调列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[ht]
\caption{MRR and Hit@10 of some representative dimensions on WN18RR.}\label{table_WN18RR}
\begin{center}
    \resizebox{.9\textwidth}{!}{
\begin{tabular}{c|l|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c}{\textbf{}}                      & \multicolumn{2}{c}{\textbf{10d}} & \multicolumn{2}{c}{\textbf{20d}} & \multicolumn{2}{c}{\textbf{40d}} & \multicolumn{2}{c}{\textbf{80d}} & \multicolumn{2}{c}{\textbf{160d}} & \multicolumn{2}{c}{\textbf{320d}} & \multicolumn{2}{c}{\textbf{640d}} \\
\midrule
\multirow{9}{*}{\textbf{TransE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\
\cline{2-16} 
                                 & DT              & .121          & .287           & .176          & .453           & .214          & .496           & .227          & .524           & .233           & .531           & .235           & .534           & \textbf{.237}  & \textbf{.537}  \\
                                 & Ext             & .125          & .298           & .172          & .423           & .199          & .468           & .213          & .495           & .225           & .515           & .226           & .521           & .237           & .537           \\
                                 & Ext-L           & .139          & .315           & .196          & .461           & .224          & .497           & .232          & .516           & .236           & \textbf{.534}  & .236           & .535           & .237           & .537           \\
                                 & Ext-V           & .139          & .309           & .198          & .458           & .222          & .494           & .234          & .525           & .236           & .532           & .236           & .536           & .237           & .537           \\
                                 & BKD             & .141          & .323           & .207          & .480           & .226          & .513           & .232          & .527           & .233           & .531           & .236           & .533           & -               & -               \\
                                 & TA              & .144          & .335           & .211          & .483           & .226          & .512           & .233          & .527           & .234           & .533           & .236           & .535           & -               & -               \\
                                 & DualDE          & .148          & .337           & .213          & .488           & .225          & .514           & \textbf{.234} & \textbf{.530}  & .235           & .533           & \textbf{.238}  & .535           & -               & -               \\
                                 & {\model}        & \textbf{.170} & \textbf{.388}  & \textbf{.219} & \textbf{.491}  & \textbf{.232} & \textbf{.518}  & .232          & .523           & \textbf{.236}  & .529           & .237           & \textbf{.536}  & .237           & .537           \\
                      %           \midrule
%\multirow{9}{*}{\textbf{SimplE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\
%\cline{2-16} 
 %                                & DT              & .061          & .126           & .257          & .372           & .316          & .389           & .382          & .446           & .409           & .459           & .417           & .474           & \textbf{.421}  & \textbf{.481}  \\
 %                                & Ext             & .004          & .007           & .051          & .107           & .160          & .249           & .219          & .314           & .357           & .401           & .407           & .451           & .421           & .481           \\
   %                              & Ext-L           & .005          & .006           & .048          & .078           & .169          & .244           & .369          & .435           & .398           & .454           & .417           & .481           & .421           & .481           \\
   %                              & Ext-V           & .004          & .006           & .047          & .076           & .246          & .317           & .368          & .402           & .398           & .461           & .413           & .472           & .421           & .481           \\
  %                               & BKD             & .075          & .156           & .285          & .381           & .343          & .399           & .394          & .450           & .414           & .468           & .418           & .475           & -               & -               \\
  %                               & TA              & .089          & .189           & .316          & .386           & .368          & .418           & .405          & .456           & .415           & .472           & .421           & .481           & -               & -               \\
  %                               & DualDE          & .083          & .175           & .328          & .388           & \textbf{.386} & .423           & .407          & .454           & \textbf{.419}  & \textbf{.475}  & \textbf{.422}  & \textbf{.483}  & -               & -               \\
 %                                & {\model}        & \textbf{.111} & \textbf{.224}  & \textbf{.335} & \textbf{.395}  & .385          & \textbf{.431}  & \textbf{.407} & \textbf{.457}  & .417           & .474           & .420           & .479           & .419           & .481           \\
                               \midrule
\multirow{9}{*}{\textbf{RotatE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\
\cline{2-16} 
                                 & DT              & .172          & .418           & .409          & .504           & .456          & .556           & .465          & .564           & .471           & .567           & .474           & .573           & \textbf{.476}  & \textbf{.575}  \\
                                 & Ext             & .299          & .378           & .379          & .464           & .437          & .516           & .458          & .544           & .467           & .549           & .471           & .552           & .476           & .575           \\
                                 & Ext-L           & .206          & .277           & .336          & .424           & .399          & .487           & .423          & .515           & .445           & \textbf{.541}  & .466           & .564           & .476           & .575           \\
                                 & Ext-V           & .261          & .377           & .304          & .433           & .337          & .471           & .366          & .497           & .416           & .532           & .451           & .561           & .476           & .575           \\
                                 & BKD             & .175          & .434           & .424          & .540           & .457          & .556           & .471          & .565           & .472           & .570           & .474           & .572           & -               & -               \\
                                 & TA              & .177          & .438           & .424          & .542           & .459          & .558           & .470          & .567           & .473           & .572           & .474           & .572           & -               & -               \\
                                 & DualDE          & .179          & .440           & .425          & .542           & .462          & .559           & \textbf{.471} & .567           & \textbf{.473}  & .573           & .475           & \textbf{.573}  & -               & -               \\
                                 & {\model}        & \textbf{.324} & \textbf{.469}  & \textbf{.456} & \textbf{.543}  & \textbf{.466} & \textbf{.561}  & .471          & \textbf{.568}  & .471           & \textbf{.574}  & \textbf{.476}  & .573           & .476           & .574          \\
                                 \midrule
                                 \multirow{9}{*}{\textbf{PairRE}} & \textit{Method} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}   & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} & \textit{MRR}    & \textit{Hit@10} \\ \cline{2-16} 
                                 & DT              & .220          & .321           & .342          & .381           & .415          & .472           & .435          & .516           & .449           & .534           & .452           & .542           & \textbf{.453}  & \textbf{.544}  \\
                                 & Ext             & .152          & .209           & .261          & .379           & .334          & .463           & .375          & .493           & .419           & .526           & .438           & .545           & .453           & .544           \\
                                 & Ext-L           & .162          & .220           & .281          & .360           & .363          & .442           & .417          & .495           & .437           & .523           & .446           & .544           & .453           & .544           \\
                                 & Ext-V           & .172          & .260           & .306          & .374           & .389          & .456           & .420          & .498           & .441           & .529           & .446           & .541           & .453           & .544           \\
                                 & BKD             & .228          & .336           & .375          & .413           & .421          & .483           & .443          & .525           & .451           & .536           & .453           & .542           & -               & -               \\
                                 & TA              & .245          & .340           & .381          & .427           & .426          & .487           & .448          & .534           & .452           & .537           & .453           & .543           & -               & -               \\
                                 & DualDE          & .242          & .336           & .377          & .424           & .428          & .495           & \textbf{.451} & .536           & \textbf{.453}  & .540           & \textbf{.454}  & \textbf{.544}  & -               & -               \\
                                 & {\model}        & \textbf{.317} & \textbf{.376}  & \textbf{.408} & \textbf{.467}  & \textbf{.433} & \textbf{.502}  & .449          & \textbf{.537}  & .451           & \textbf{.541}  & .451           & .542           & .451           & .542          
                                 \\
                                 \bottomrule

                                 
\end{tabular}
}
\end{center}
\end{table*}


==> table/table-para_effi-cd-yg.tex <==
\setlength\tabcolsep{4pt}%列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[h]
\setlength{\belowcaptionskip}{0.05cm}
\caption{Link prediction results on CoDEx-L and YAGO3-10.}
\label{table_lp_cd_yg}
\begin{center}
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lccccc|ccccc}
\toprule
                  & \multicolumn{5}{c}{CoDEx-L}                                                        & \multicolumn{5}{c}{YAGO3-10}                                                       \\
                  & \textit{Dim} & \textit{\#P(M)} & \textit{MRR}   & \textit{Hit@10} & \textit{Effi}  & \textit{Dim} & \textit{\#P(M)} & \textit{MRR}   & \textit{Hit@10} & \textit{Effi}  \\
                  \midrule
RotatE*           & 500          & 78              & 0.258          & 0.387           & 0.003          & 500          & 123.2           & 0.495          & 0.670           & 0.004          \\
RotatE*           & 25           & 3.8             & 0.196          & 0.322           & 0.052          & 20           & 4.8             & 0.121          & 0.262           & 0.025          \\
NodePiece+RotatE* & 100          & 3.6             & 0.190          & 0.313           & 0.053          & 100          & 4.1             & 0.247          & 0.488           & 0.06           \\
EARL+RotatE       & 100          & \text{2.1}    & 0.238          & \text{0.390}  & \text{0.113} & 100          & \text{3}      & 0.302          & 0.498           & \text{0.101} \\
\model            & \text{20}  & 3.1             & \text{0.243} & 0.385           & 0.078          & \text{20}  & 4.9             & \text{0.313} & \text{0.528}  & 0.064         \\ \bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> table/table-para_effi-fb-wn.tex <==
%\setlength\tabcolsep{4pt}%列距
%\renewcommand\arraystretch{.9}%行距 
\begin{table*}[h]
\setlength{\belowcaptionskip}{0.05cm}
\caption{Link prediction results on WN18RR and FB15K237.}
\label{table_lp_wn_fb}
\begin{center}
    \resizebox{.8\textwidth}{!}{
\begin{tabular}{lccccc|ccccc}
\toprule
                  & \multicolumn{5}{c}{FB15K237}                                                       & \multicolumn{5}{c}{WN18RR}                                                         \\
                  & \textit{Dim} & \textit{\#P(M)} & \textit{MRR}   & \textit{Hit@10} & \textit{Effi}  & \textit{Dim} & \textit{\#P(M)} & \textit{MRR}   & \textit{Hit@10} & \textit{Effi}  \\
                  \midrule
RotatE*           & 1000         & 29.3           & 0.336          & 0.532            & 0.011          & 500          & 40.6           & 0.508          & 0.612            & 0.013          \\
RotatE*           & 100          & 2.9            & 0.296          & 0.473            & 0.102          & 50           & 4.1            & 0.411          & 0.429            & 0.100          \\
NodePiece+RotatE* & 100          & 3.2            & 0.256          & 0.420            & 0.080          & 100          & 4.4            & 0.403          & 0.515            & 0.092          \\
EARL+RotatE       & 150          & 1.8            & 0.310          & 0.501            & 0.172          & 200          & 3.8            & 0.440          & 0.527            & 0.116          \\
\model            & \text{40}  & \text{1.2}   & \text{0.318} & \text{0.504}   & \text{0.265} & \text{40}  & \text{3.2}   & \text{0.466} & \text{0.561}   & \text{0.146}\\ \bottomrule
\end{tabular}
}
\end{center}
\end{table*}

